Benchmarking Model-Based Reinforcement Learning

Model-based reinforcement learning (MBRL) is widely seen as having the potential to be significantly more sample efficient than model-free RL. However, research in model-based RL has not been very standardized. It is fairly common for authors to experiment with self-designed environments, and there are several separate lines of research, which are sometimes closed-sourced or not reproducible. Accordingly, it is an open question how these various existing MBRL algorithms perform relative to each other. To facilitate research in MBRL, in this paper we gather a wide collection of MBRL algorithms and propose over 18 benchmarking environments specially designed for MBRL. We benchmark these algorithms with unified problem settings, including noisy environments. Beyond cataloguing performance, we explore and unify the underlying algorithmic differences across MBRL algorithms. We characterize three key research challenges for future MBRL research: the dynamics bottleneck, the planning horizon dilemma, and the early-termination dilemma. Finally, to maximally facilitate future research on MBRL, we open-source our benchmark in http://www.cs.toronto.edu/~tingwuwang/mbrl.html.

==> trash_bin.tex <==
\begin{table}[!t]
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\toprule % OliveGreen % OrangeRed % MidnightBlue 
&HalfCheetah & HalfCheetah,\,$\sigma_o = 0.1$    & HalfCheetah,\,$\sigma_o = 0.01$ & HalfCheetah,\,$\sigma_a = 0.1$  & HalfCheetah,\,$\sigma_a = 0.03$\\
\midrule
% Random  & -288.3 $\pm$ 65.8     & -288.3 $\pm$ 65.8   & -288.3 $\pm$ 65.8   & -288.3 $\pm$ 65.8     & -288.3 $\pm$ 65.8     & -202.6 $\pm$ 249.3  & -202.6 $\pm$ 249.3   & -202.6 $\pm$ 249.3 & 38.4 $\pm$ 32.5     & 38.4 $\pm$ 32.5      & 38.4 $\pm$ 32.5    \\
iLQR    & 2142.6 $\pm$ 137.7    & \color{OrangeRed}-25.3 $\pm$ 127.5   & \color{OrangeRed}187.2 $\pm$ 102.9   & \color{OrangeRed}261.2 $\pm$ 106.8     & \color{OrangeRed}310.1 $\pm$ 112.6     \\
GT-PETS & 14777.2 $\pm$ 13964.2 & \color{OrangeRed}1638.5 $\pm$ 188.5  & \color{OrangeRed}9226.5 $\pm$ 8893.4 & \color{OrangeRed}11484.5 $\pm$ 12264.7 & \color{OrangeRed}13160.6 $\pm$ 13642.6  \\
% GT-RS   & 815.7 $\pm$ 38.5      & \color{OrangeRed}6.6 $\pm$ 52.5      & \color{OrangeRed}493.3 $\pm$ 38.3    & \color{OrangeRed}604.8 $\pm$ 42.7      & \color{OrangeRed}645.7 $\pm$ 39.6       \\
RS      & 421.0 $\pm$ 55.2      & \color{OrangeRed}146.2 $\pm$ 19.9    & \color{OliveGreen}423.1 $\pm$ 28.7    & \color{OliveGreen}445.8 $\pm$ 19.2      & \color{OliveGreen}442.3 $\pm$ 26.0       \\
% MB-MF    & 126.9 $\pm$ 72.7      & \color{OliveGreen}146.1 $\pm$ 87.8    & \color{OliveGreen}232.1 $\pm$ 122.0   & \color{OliveGreen}184.0 $\pm$ 148.9     & \color{OliveGreen}257.0 $\pm$ 96.6     \\
PETS    & 2795.3 $\pm$ 879.9    & \color{OrangeRed}1879.5 $\pm$ 801.5  & \color{OrangeRed}2410.3 $\pm$ 844.0  & \color{OrangeRed}2427.5 $\pm$ 674.1    & \color{OrangeRed}2427.2 $\pm$ 1118.6   \\
% PETS-RS & 966.9 $\pm$ 471.6     & \color{OrangeRed}217.0 $\pm$ 193.4   & \color{OrangeRed}814.9 $\pm$ 678.6   & \color{OliveGreen}1128.6 $\pm$ 674.2    & \color{OliveGreen}1017.5 $\pm$ 734.9    \\
ME-TRPO  & 2283.7 $\pm$ 900.4    & \color{OrangeRed}409.4 $\pm$ 834.2   & \color{OrangeRed}1396.9 $\pm$ 834.8  & \color{OrangeRed}1319.8 $\pm$ 698.0    & \color{OrangeRed}2122.9 $\pm$ 889.1   \\
% GPS     & 52.3 $\pm$ 41.7       & \color{OrangeRed}-6.8 $\pm$ 13.6     & \color{OliveGreen}175.2 $\pm$ 169.4   & \color{OrangeRed}41.6 $\pm$ \color{OrangeRed}45.7       & \color{OliveGreen}94.0 $\pm$ 57.0       \\
% PILCO   & -41.9 $\pm$ 267.0 & \color{OrangeRed}-282.0 $\pm$ 258.4 & \color{OrangeRed}-275.4 $\pm$ 164.6 & \color{OrangeRed}-175.6 $\pm$ 284.1 & \color{OrangeRed}-260.8 $\pm$ 290.3 \\
SVG     &  336.6 $\pm$ 387.6 & \color{OrangeRed}0.1 $\pm$ 271.3 & \color{OrangeRed}240.8 $\pm$ 236.6 & \color{OrangeRed}163.5 $\pm$ 338.6 & \color{OrangeRed}21.9 $\pm$ 81.0  \\
MB-MPO  & 3639.0 $\pm$ 1185.8  &  \color{OrangeRed}2356.4 $\pm$ 734.4  &  \color{OrangeRed}3635.5 $\pm$ 1486.8  &  \color{OrangeRed}3372.9 $\pm$ 1373 & \color{OliveGreen}3718.7 $\pm$ 922.3 \\
SLBO &  1097.7 $\pm$ 166.4	& \color{OrangeRed}212.5 $\pm$ 279.6	& \color{OliveGreen}1244.8 $\pm$ 604.0 & \color{OliveGreen}1593.2 $\pm$ 265.0 &	\color{OrangeRed}731.1 $\pm$ 215.8\\\bottomrule
% PPO     & 17.2 $\pm$ 84.4       & \color{OrangeRed}-113.3 $\pm$ 92.8   & \color{OrangeRed}-83.1 $\pm$ 117.7   & \color{OrangeRed}-28.0 $\pm$ 54.1      & \color{OrangeRed}-35.5 $\pm$ 87.8    \\
% TRPO    & -12.0 $\pm$ 85.5      & \color{OrangeRed}-146.0 $\pm$ 67.4   & \color{OliveGreen}9.4 $\pm$ 57.6      & \color{OrangeRed}-32.7 $\pm$ 110.9     & \color{OrangeRed}-70.9 $\pm$ 71.9   \\
% TD3     & 3614.3 $\pm$ 82.1     & \color{OrangeRed}895.7 $\pm$ 61.6    & \color{OrangeRed}817.3 $\pm$ 11.0    & \color{OliveGreen}4256.5 $\pm$ 117.4    & \color{OliveGreen}3941.8 $\pm$ 61.3     \\
% SAC     & 4000.7 $\pm$ 202.1    &  \color{OrangeRed}1146.7 $\pm$ 67.9   &  \color{OrangeRed}3869.2 $\pm$ 88.2   &  \color{OrangeRed}3530.5 $\pm$ 67.8     &  \color{OrangeRed}3708.1 $\pm$ 96.2   \\\bottomrule
\end{tabular}}

\vspace{0.1cm}
\caption{The performance of each algorithm in noisy environments. The red color indicates a decrease of performance while green indicates increase of performance.}\label{table:noisy_env}
\vspace{-.75 cm}
\end{table}

% the intros
\iffalse
Reinforcement learning (RL) algorithms are most commonly classified in two categories: model-free RL (MFRL) and model-based RL (MBRL). 
While model-free algorithms have achieved success in areas including robotics~\cite{lillicrap2015continuous,ppo,deepmindppo,andrychowicz2018learning}, video-games~\cite{dqn, mnih2016asynchronous}, and motion animation~\cite{peng2018deepmimic},
they are data inefficient, which limits their applications in simulated domains.
By learning a model of the environment,
model-based methods are able to obtain substantially lower sample complexity. 
However, modelling errors or model-bias~\cite{deisenroth2011pilco} cripple effectiveness of these algorithms,
resulting in sub-optimal behaviour.
Recently, probabilistic models or ensembles, which better capture model uncertainty,
have resulted in algorithms that are able to match the model-free asymptotic performance while using much fewer samples~\cite{kurutach2018model, chua2018deep}.

% However, the lack of a standardized implementations and environments for model-based RL makes it difficult to quantify scientific progress.
MFRL has greatly benefited from the introduction of benchmarking code bases and environments such as rllab~\cite{duan2016benchmarking},
OpenAI Gym~\cite{gym} and Deepmind Control Suite~\cite{tassa2018deepmind},
where the latter two have been the de facto benchmarking platforms.
% \ignasi{It would be amazing if we could throw some data here!}\tingwu{you mean citations for paper using gym and dm control?}
Benchmarking platforms have played an important role in RL,
as well as other areas such as computer vision~\cite{deng2009imagenet,lin2014microsoft},
machine translation and speech recognition.
% whose notable examples include ImageNet~\cite{deng2009imagenet}, 
% \ignasi{TODO: add benchmarks with citation! Maybe say that benchmarks are even created nowadays to work on specific problems (for instance all the challenges that companies create)}.

Despite the recent impressive progress in MBRL,
the actual performance of these algorithms remains unclear.
Large implementation differences between algorithms,
lack of open-source code,
and the difficulty to reproduce results makes it difficult for researchers to compare novel algorithms against prior work.
The lack of proper comparison is exacerbated by modifications of the standard model-free environments to hold the assumptions of the proposed methods.
Modification of the reward functions, shortening of the horizons, or pre-processing of the observations are standard techniques in model-based research. We argue that systematic evaluation and comparison will not only further our understanding of the strengths of existing algorithms, but also reveal their limitations and suggest directions for future research.

In this paper, we propose 18 environments, based on the standard OpenAI Gym~\cite{gym} ones, and we benchmark the performance of 11 different model-based algorithms. The environments are designed to hold the common assumptions in model-based algorithms, such as differential reward function, and present standardized observation space and task horizon. This environments range from simple and usually tested on, such as cart-pole, to complex and never tested on before domains such as humanoid. The performance of the algorithms is further evaluated when stochasticity is introduced in the observations and actions.

Our evaluation identifies the main causes of the gap between model-based and model-free methods as follows. 1) \emph{Dynamics bottleneck}: Algorithms with learned dynamics are stuck at a performance local minima significantly worse than their performance with ground-truth dynamics. 2) \emph{Planning horizon dilemma},
while increasing planning horizon provides more accurate reward estimation,
it suffers performance drop due to the curve of dimensionality and modelling errors. 3)
\emph{Early-termination dilemma},
early termination is commonly used in model-free for more directed exploration resulting in faster learning, however, the performance gain is not observed in MB algorithms,
which limits the effectiveness in complex environments.
\fi

% \fi
% In practice, the dynamics is either unknown or inaccurate,
% and the modelling error of the dynamics cripples the effectiveness of MBRL algorithms in both sample efficiency and asymptotic performance.
% Very recently, neural network ensembles~\cite{kurutach2018model},
% or probabilistic ensembles with trajectory sampling~\cite{chua2018deep} are respectively used in MBRL.
% By capturing the uncertainty of the environment,
% MRBL algorithms start to match state-of-the-art MFRL algorithms in complex environments such as Cheetah,
% while retaining the low sample complexity.

% Model-based approaches tended to converge at a performance level well below their model-free counterparts~\cite{nagabandi2017neural}.
%\ignasi{May be we should talk here at some point of model-bias, and the next line that MB that with better characterization of the uncertainty, current algos do not suffer that much from it allowing allowing them to achieve the same performance as MF.}
% However,
% with better modelling methods of the environment,
% recent works have developed algorithms that are able to attain asymptotic model-free performance while retaining the low sample complexity~\cite{clavera2018mbmpo, chua2018deep}.

\iffalse
%Second intro
Reinforcement learning (RL) algorithms are most commonly classified in two categories: model-free RL (MFRL) and model-based RL (MBRL). While model-free algorithms have achieved success in robotics~\cite{lillicrap2015continuous,ppo,deepmindppo,andrychowicz2018learning}, video-games~\cite{dqn, mnih2016asynchronous}, and motion animation~\cite{peng2018deepmimic}; they are data inefficient, which limits their application to simulated domains. By learning a model of the environment, model-based methods are able to obtain substantially lower sample complexity. 
However, modelling errors cripple effectiveness of these algorithms resulting in sub-optimal behaviour, problem known as model-bias~\cite{deisenroth2011pilco}. Recently, better characterization of the model uncertainty's by the means of probabilistic models or ensembles has resulted in algorithms that are able to match the model-free asymptotic performance~\cite{kurutach2018model, chua2018deep}.

Despite the recent impressive results on model-based RL, the actual applicability of these algorithms remains unclear. 
Different lines of research usually evaluate the performance of their algorithms on self-designed environments.
Pre-processing of the observations, modification of the reward functions,
or using different horizons are standard techniques to favor the proposed algorithms.
Furthermore, due to the large implementation differences between algorithms, lack of open-source code, and the difficulty to reproduce results, model-based research does not tend to compare against prior methods.
At the same time, model-free RL research has been greatly benefited by the introduction of benchmarking code bases and environments such as rllab~\cite{duan2016benchmarking},
OpenAI Gym~\cite{gym} and Deepmind Control Suite~\cite{tassa2018deepmind},
where the latter two have been the de facto benchmarking platforms. The lack of a standardized implementations and environments for model-based RL makes it difficult to quantify scientific progress. Systematic evaluation and comparison will not only further our understanding of the strengths of existing algorithms, but also reveal their limitations and
suggest directions for future research.

In this paper, we benchmark the performance of 11 model-based algorithms across 18 standard environments and 8 noisy environments. These environments range from the simple domains model-based is usually tested on, such as cart-pole, to complex domains such as humanoid. We also evaluate the performance drop when stochasticity is introduced in the observations and actions. Finally, based on the empirical results, we identify the main causes of the gap between model-based and model-free methods as follows. (1) \emph{Dynamics bottleneck}: Algorithms with learned dynamics are stuck at a performance local minima significantly worse than their performance with ground-truth dynamics. (2) \emph{Planning horizon dilemma},
while increasing planning horizon provides more accurate reward estimation,
it suffers performance drop due to the curve of dimensionality and modelling errors. (3)
\emph{Early-termination dilemma},
early termination is commonly used in model-free for more directed exploration resulting in faster learning, however, the performance gain is not observed in MB algorithms,
which limits the effectiveness in complex environments.
\fi
\iffalse
\ignasi{The intro above is mine.}


% The lack of a standardized and challenging testbed for reinforcementlearning and continuous control makes it difficult to quan-tify scientific progress. Systematic evaluation and compar-ison will not only further our understanding of the strengthsof existing algorithms, but also reveal their limitations andsuggest directions for future research.
% Explain what's wrong with this problems.

% How previous benchmarks have veen useful.

% \fi
Model-free reinforcement learning (MFRL) has made numerous successes in applications such as playing video games,
robot hand manipulation and character animation~\cite{dqn, mnih2016asynchronous,lillicrap2015continuous,ppo,deepmindppo,peng2018deepmimic,andrychowicz2018learning}. 
One major drawback of MFRL is its sample inefficiency,
where millions of interaction time-steps are sometimes needed to solve one single task.
Some of the latest attempts include~\cite{haarnoja2018soft, fujimoto2018addressing},
which are able to increase inefficiency by orders of magnitude.
But still, the sample inefficiency prohibits the use of MFRL in many real-life applications.

Model-based reinforcement learning (MBRL) on the other hand,
% which models the dynamics function of the agent,
is believed by many to potentially have better sample efficiency.
With dynamics function, the agent can increase sample efficiency and performance by,
for example, bootstrapping value estimation or online re-planning.
However, for most of the applications,
the dynamics is either unknown or inaccurate,
and the modelling error of the dynamics cripples the effectiveness of MBRL algorithms in both sample efficiency and asymptotic performance.
Very recently, neural network ensembles~\cite{kurutach2018model},
or probabilistic ensembles with trajectory sampling~\cite{chua2018deep} are respectively used in MBRL.
By capturing the uncertainty of the environment,
for the first time, MRBL algorithms start to match state-of-the-art MFRL algorithms in complex environments such as Cheetah,
yet with much less data samples.

MFRL Research has been accelerated by the introduction of bench-marking environments such as rllab~\cite{duan2016benchmarking},
OpenAI Gym~\cite{gym} and Deepmind Control Suite~\cite{tassa2018deepmind},
where the latter two have been the de facto bench-marking platforms for most of the MFRL algorithms.
However, MBRL algorithms, although long studied,
are usually not tested on a general bench-marking platform and sometimes not reproducible.
% which makes it hard to evaluate the algorithms.
% use differnt env
% hacks (length, preprocessing)
% not reproducible
Different lines of research usually evaluate the performance on self-designed environments,
and often does not compare with each other.
For example, ~\cite{deisenroth2011pilco, deisenroth2015gaussian, kamthe2017data} experiment majorly only with Cart-pole or Pendulum,
and a separate line of research~\cite{levine2015learning, zhang2016learning, finn2016guided, montgomery2016guided} experiment with a collection of environments based on ROS~\cite{ros} and MuJoCo~\cite{2012mujoco}.
It is also very common in existing research to customize the environments in favor of the proposed algorithms.
For exmaple, in~\cite{kurutach2018model,luo2018algorithmic},
episode length is much shorter than the one used in original environments.
In~\cite{chua2018deep}, additional observation pre-processing is applied on the environments.
% In~\cite{finn2016guided, montgomery2016guided},
% there is no randomness of the initial states for the simulated environments across iterations.
Some of the algorithms are not open-sourced and difficult to reproduce in practice~\cite{heess2015learning, tassa2012synthesis}.

In this paper,
we proposed 18 standard environments and 8 noisy environments,
from simple Pendulum with episode length of 200,
to complex Humanoid with maximum episode length of 1000.
We fairly bench-mark a wide collection of existing MBRL algorithms across different random seeds,
without over-exhaustive hyper-parameter search or additional environment processing.

We further propose the following observations from empirical results.
First of all, MBRL algorithms with learned dynamics are stuck at a performance local-minima significantly worse than their performance with ground-truth dynamics,
% and training for longer episodes does not increase the performance,
which we name as \emph{dynamics bottleneck}.
The second observation is called \emph{planning horizon dilemma}.
While increasing planning horizon provides more accurate reward estimation,
it suffers performance drop due to the curve of dimentionality and modelling errors.
The last observation is called \emph{early-termination dilemma}.
Early termination is commonly used in MFRL to more efficiently collect important data samples.
But the same performance gain is not observed in MBRL algorithms,
which limits the effectiveness of MBRL algorithms in more complex environments.
% These observations potentially propose important requests of research for MBRL.
% , which we believe will inspire future research in MBRL.
% The problems of MBRL environments
% the following commented paragraphs was the first edition of the intro.
% it has too much related work content, but was not able to illustrate why MB is the future way to go
\ignasi{The introduction feels more like an amazing related work section. We need to motivate more the reason why are we doing this benchmark, and remove all the names of the algorithms in the intro.

I see it like this:
\begin{enumerate}
    \item Motivate model-based. And get people excited about the current state-of-the art in model-based RL: It's the first time we have MB algorithms that achieve the same performance than MF with way less data.
    \item Second paragraph: motivate the problem. All these results are amazing but all these algorihtms are tested in different environments, they use different hacks, different horizons, etc...
    \item Explain what we are doing
    \item Summarize our findings.
\end{enumerate}
}

The recent progress in reinforcement learning (RL) has been accelerated by the progress of neural networks, and especially deep neural networks.
Among the progress, model-free reinforcement learning (MFRL) algorithms, which do not model the dynamics,
has been most successful in the past few years.

\ignasi{We do not need to discuss all this bulk of work on model-free. Just mention the ones we compared because they are the state-of-the-art and that they achieve better asymptotic performance than model-based (so, just a small paragraph on model-free in the end.}
Some of the early successful attempts of MFRL applications date back to Atari games with image input,
where researchers propose DQN~\cite{dqn} that applies a convolutional neural network on Q-learning.
Following this line of research, algorithms such as A3C~\cite{mnih2016asynchronous}, ACER~\cite{wang2016sample} and ACKTR~\cite{wu2017scalable} were further proposed.
In locomotion control,
trust region methods~\cite{trpo,ppo,deepmindppo,peng2018deepmimic,andrychowicz2018learning} and policy gradient methods~\cite{silver2014deterministic, lillicrap2015continuous, barth2018distributed} have been demonstrated capable of solving complex tasks such as humanoid control~\cite{peng2018deepmimic} and robot hand manipulation.
% In trust region methods, including TRPO~\cite{trpo}, PPO~\cite{ppo,deepmindppo},
% agents can solve complex tasks such as humanoid control~\cite{peng2018deepmimic} and robot hand manipulation~\cite{andrychowicz2018learning}.
% Policy gradient methods, which includes DPG, DDPG, D4PG~\cite{silver2014deterministic, lillicrap2015continuous, barth2018distributed}, have comparable performance to trust region methods.
Being recently proposed,
SAC~\cite{haarnoja2018soft} and TD3~\cite{fujimoto2018addressing}
are considered by many to be the state-of-the-art locomotion control algorithms,
which greatly increase the sample efficiency of model-free algorithms.
% which combines actor-critic and maximum entropy objective,
% which is a variant of policy gradient methods, 
MFRL Research has been accelerated by the introduction of bench-marking environments such as rllab~\cite{duan2016benchmarking},
OpenAI Gym~\cite{gym} and Deepmind Control Suite~\cite{tassa2018deepmind},
where the latter two have been the de facto bench-marking platforms for most of the MFRL algorithms.
\tingwu{Make the related work on MBRL shorter. Talk more about the problems of MB environments and benchmarking}
While MFRL has been very successful, it requires a huge amount of samples,
which limits its real-life applications.
To increase sample efficiency, a lot of research effort has also been spent on model-based reinforcement learning (MBRL).
% There are different ways of utilizing the learned dynamics function.
Dyna is among the early attempts of combining learned dynamics and RL agents~\cite{sutton1990integrated, sutton1991dyna, sutton1991planning}.
In Dyna, the agent learns a world model or dynamics function, and generate hypothetical experience to train a reinforcement learning controller.
Recently with the progress of model-free controllers,
modern variants of Dyna such as ME-TRPO~\cite{kurutach2018model} and SLBO~\cite{luo2018algorithmic} are proposed,
where the authors uses neural networks to learn the dynamics and train a policy network with TRPO~\cite{trpo} on data generated by the learned dynamics.
Efficient as ME-TRPO and SLBO can be,
they receive some doubts on its stableness and scalability on tasks with longer episode.

Some other algorithms use dynamics function to perform more efficient policy search which optimizes the objective function.
% using back-propagation through the dynamics network and directly into the policy network.
In PILCO~\cite{deisenroth2011pilco, deisenroth2015gaussian, kamthe2017data},
the authors use Gaussian process to model the dynamics.
By computing the analytic expected reward as a function of policy parameters,
PILCO can directly optimize the policy network.
While PILCO is efficient at solving some simple environments,
the use of Gaussian process makes PILCO very vulnerable to the curse of dimensionality.
In SVG~\cite{heess2015learning},
instead of using Gaussian process, the authors simply use fully connected neural network.
Reparameterization trick is used so that the computation graph is still back-propagatable even when the controllers are stochastic.
SVG is more scalable than PILCO,
but SVG does not have open-sourced code-bases,
and in practice some researchers claim that it is not stable in their implementation~\cite{kurutach2018model}.
Policy can also be optimized by dynamic programming.
GPS uses iLQR, iLQG or DDG~\cite{li2004iterative, todorov2005generalized, tassa2012synthesis, tassa2014ddp} to optimize time-dependent controllers and distill those controllers into a neural network.
% iLQG assumes the dynamics is linear and the reward function is quadratic.
Different variants of GPS, which includes~\cite{levine2014learning, levine2015learning, zhang2016learning, finn2016guided, montgomery2016guided, chebotar2017path, zhang2018solar}, are applied to different problem domains with different optimization techniques.
But in general GPS has not been compared with recent reinforcement learning controllers.

Dynamics function can also be used in online planning or model-predictive control.
If the dynamics function is known, iLQG is used to update the controller after every time-step~\cite{tassa2012synthesis}.
More commonly, in random sampling shooting or random shooting algorithms~\cite{richards2005robust, rao2009survey},
dynamics are used to predict future trajectories given randomly generated control sequences.
Monte-carlo tree search in planning is very famous for its use in AlphaGo~\cite{alphago,silver2017mastering, guez2018learning}.
In locomotion control problems where the dynamics is unknown,
random shooting algorithms generally cannot achieve the same asymptotic performance of MF controllers.
In MBMF~\cite{nagabandi2017neural},
the authors use model-free algorithms to fine-tune the random shooting controllers.
Recently, by applying probabilistic ensemble on the dynamics and combining CEM~\cite{de2005tutorial,botev2013cross} in the random shooting,
PETS~\cite{chua2018deep} achieve comparable performance to MF algorithms on Cheetah.
However, PETS is only tested on 4 environments with human pre-processed observation functions.
Instead of random shooting, in~\cite{henaff2017model, srinivas2018universal},
gradient based online-planning is also used.

At the same time, many algorithms use dynamics function to provide better estimation of value function or speed up the training of model-free controllers~\cite{gu2016continuous, alphago, silver2017mastering, racaniere2017imagination, feinberg2018model, buckman2018sample}.
For observation of higher dimension such as images,
VAE~\cite{kingma2013auto} has been used to encode raw observation into latent space,
which were shown in~\cite{ha2018recurrent, ha2018world, hafner2018learning, zhang2018solar, kaiser2019model}.
In general these algorithms can be regarded as successful variants of the model-free or model-based algorithms they built upon,
and we do not specifically study in this paper.

% To sum up, there are a wide range of model-based algorithms with different ways of utilizing the dynamics.
To sum up previous research and facilitate future research,
we perform a detailed bench-marking in this paper.
We proposed 18 standard environments and 8 noisy environments,
and examine a wide collection of existing MBRL algorithms.
We further propose four observations: dynamics bottleneck, noise stability, planning depth dilemma and early-termination dilemma, which we believe will inspire future research in MBRL.
\fi





























\begin{table}[!ht]
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
\toprule % OliveGreen % OrangeRed % MidnightBlue \color{MidnightBlue}
&Cheetah & Cheetah-O-01    & Cheetah-O-001 & Cheetah-A-01  & Cheetah-A-003   & Pendulum        & Pendulum-O-01 & Pendulum-O-001 & Cartpole     & Cartpole-O-01 & Cartpole-O-001        \\
\midrule
% Random  & -288.3 $\pm$ 65.8     & -288.3 $\pm$ 65.8   & -288.3 $\pm$ 65.8   & -288.3 $\pm$ 65.8     & -288.3 $\pm$ 65.8     & -202.6 $\pm$ 249.3  & -202.6 $\pm$ 249.3   & -202.6 $\pm$ 249.3 & 38.4 $\pm$ 32.5     & 38.4 $\pm$ 32.5      & 38.4 $\pm$ 32.5    \\
iLQR    & \color{MidnightBlue}2142.6 $\pm$ 137.7    & \color{OrangeRed}-25.3 $\pm$ 127.5   & \color{OrangeRed}187.2 $\pm$ 102.9   & \color{OrangeRed}261.2 $\pm$ 106.8     & \color{OrangeRed}310.1 $\pm$ 112.6     & \color{MidnightBlue}160.8 $\pm$ 29.8    & \color{OrangeRed}-357.9 $\pm$ 251.9   & \color{OrangeRed}-2.2 $\pm$ 166.5   & \color{MidnightBlue}200.3 $\pm$ 0.6     & \color{OrangeRed}197.8 $\pm$ 2.9      & \color{OliveGreen}200.4 $\pm$ 0.7    \\
GT-PETS & \color{MidnightBlue}14777.2 $\pm$ 13964.2 & \color{OrangeRed}1638.5 $\pm$ 188.5  & \color{OrangeRed}9226.5 $\pm$ 8893.4 & \color{OrangeRed}11484.5 $\pm$ 12264.7 & \color{OrangeRed}13160.6 $\pm$ 13642.6 & \color{MidnightBlue}170.5 $\pm$ 35.2    & 171.4 $\pm$ 26.2     & \color{OrangeRed}157.3 $\pm$ 66.3   & \color{MidnightBlue}200.9 $\pm$ 0.1     & 199.5 $\pm$ 1.2      & 200.9 $\pm$ 0.1    \\
GT-RS   & \color{MidnightBlue}815.7 $\pm$ 38.5      & \color{OrangeRed}6.6 $\pm$ 52.5      & \color{OrangeRed}493.3 $\pm$ 38.3    & \color{OrangeRed}604.8 $\pm$ 42.7      & \color{OrangeRed}645.7 $\pm$ 39.6      & \color{MidnightBlue}171.5 $\pm$ 31.8    & \color{OrangeRed}125.2 $\pm$ 40.3     & \color{OrangeRed}157.8 $\pm$ 39.1   & \color{MidnightBlue}201.0 $\pm$ 0.0     & 200.2 $\pm$ 0.3      & 201.0 $\pm$ 0.0    \\
RS      & \color{MidnightBlue}421.0 $\pm$ 55.2      & \color{OrangeRed}146.2 $\pm$ 19.9    & \color{OliveGreen}423.1 $\pm$ 28.7    & \color{OliveGreen}445.8 $\pm$ 19.2      & \color{OliveGreen}442.3 $\pm$ 26.0      & \color{MidnightBlue}164.4 $\pm$ 9.1     & \color{OrangeRed}154.5 $\pm$ 12.9     & 160.1 $\pm$ 6.7    & \color{MidnightBlue}201.0 $\pm$ 0.0     & 197.7 $\pm$ 4.5      & 200.9 $\pm$ 0.0    \\
MB-MF    & \color{MidnightBlue}126.9 $\pm$ 72.7      & \color{OliveGreen}146.1 $\pm$ 87.8    & \color{OliveGreen}232.1 $\pm$ 122.0   & \color{OliveGreen}184.0 $\pm$ 148.9     & \color{OliveGreen}257.0 $\pm$ 96.6      & \color{MidnightBlue}157.5 $\pm$ 13.2    & \color{OliveGreen}162.8 $\pm$ 14.7     & \color{OliveGreen}165.9 $\pm$ 8.5    & \color{MidnightBlue}199.7 $\pm$ 1.2     & \color{OrangeRed}152.3 $\pm$ 48.3     & \color{OrangeRed}137.9 $\pm$ 48.5   \\
PETS    & \color{MidnightBlue}2795.3 $\pm$ 879.9    & \color{OrangeRed}1879.5 $\pm$ 801.5  & \color{OrangeRed}2410.3 $\pm$ 844.0  & \color{OrangeRed}2427.5 $\pm$ 674.1    & \color{OrangeRed}2427.2 $\pm$ 1118.6   & \color{MidnightBlue}167.4 $\pm$ 53.0    & \color{OliveGreen}174.7 $\pm$ 27.8     & 166.7 $\pm$ 52.0   & \color{MidnightBlue}199.5 $\pm$ 3.0     & \color{OrangeRed}156.6 $\pm$ 50.3     & 196.1 $\pm$ 5.1    \\
PETS-RS & \color{MidnightBlue}966.9 $\pm$ 471.6     & \color{OrangeRed}217.0 $\pm$ 193.4   & \color{OrangeRed}814.9 $\pm$ 678.6   & \color{OliveGreen}1128.6 $\pm$ 674.2    & \color{OliveGreen}1017.5 $\pm$ 734.9    & \color{MidnightBlue}167.9 $\pm$ 35.8    & \color{OrangeRed}148.0 $\pm$ 58.6     & \color{OrangeRed}113.6 $\pm$ 124.1  & \color{MidnightBlue}195.0 $\pm$ 28.0    & 192.3 $\pm$ 20.6     & 200.8 $\pm$ 0.2    \\
ME-TRPO  & \color{MidnightBlue}2283.7 $\pm$ 900.4    & \color{OrangeRed}409.4 $\pm$ 834.2   & \color{OrangeRed}1396.9 $\pm$ 834.8  & \color{OrangeRed}1319.8 $\pm$ 698.0    & \color{OrangeRed}2122.9 $\pm$ 889.1    & \color{MidnightBlue}177.3 $\pm$ 1.9     & 173.3 $\pm$ 3.2      & 173.7 $\pm$ 4.8    & \color{MidnightBlue}160.1 $\pm$ 69.1    & \color{OliveGreen}174.9 $\pm$ 21.9     & 165.9 $\pm$ 58.5   \\
GPS     & \color{MidnightBlue}52.3 $\pm$ 41.7       & \color{OrangeRed}-6.8 $\pm$ 13.6     & \color{OliveGreen}175.2 $\pm$ 169.4   & \color{OrangeRed}41.6 $\pm$ \color{OrangeRed}45.7       & \color{OliveGreen}94.0 $\pm$ 57.0       & \color{MidnightBlue}162.7 $\pm$ 7.6     & 162.2 $\pm$ 4.5      & 168.9 $\pm$ 6.8    & \color{MidnightBlue}14.4 $\pm$ 18.6     & \color{OrangeRed}-479.8 $\pm$ 859.7   & \color{OrangeRed}-22.7 $\pm$ 53.8   \\
PILCO   & \color{MidnightBlue}-41.9 $\pm$ 267.0 & \color{OrangeRed}-282.0 $\pm$ 258.4 & \color{OrangeRed}-275.4 $\pm$ 164.6 & \color{OrangeRed}-175.6 $\pm$ 284.1 & \color{OrangeRed}-260.8 $\pm$ 290.3 & \color{MidnightBlue}-132.6 $\pm$ 410.1 & \color{OrangeRed}-211.6 $\pm$ 272.1 & \color{OliveGreen}168.9 $\pm$ 30.5 & \color{MidnightBlue}-1.9 $\pm$ 155.9 & 139.9 $\pm$ 54.8 & -2060.1 $\pm$ 14.9 \\
SVG     &  \color{MidnightBlue}336.6 $\pm$ 387.6 & \color{OrangeRed}0.1 $\pm$ 271.3 & \color{OrangeRed}240.8 $\pm$ 236.6 & \color{OrangeRed}163.5 $\pm$ 338.6 & \color{OrangeRed}21.9 $\pm$ 81.0 & \color{MidnightBlue}141.4 $\pm$ 62.4 & \color{OrangeRed}86.7 $\pm$ 34.6 & \color{OrangeRed}78.8 $\pm$ 73.2 & \color{MidnightBlue}82.1 $\pm$ 31.9 & \color{OliveGreen}119.2 $\pm$ 46.3 & \color{OliveGreen}106.6 $\pm$ 42.0\\
MB-MPO  &                 &               &               &                 &                 &               &                &              &               &                &              \\
SLBO & \color{MidnightBlue} 1097.7 $\bm$ 166.4	& \color{OrangeRed}212.5 $\bm$ 279.6	& \color{OliveGreen}1244.8 $\bm$ 604.0 & \color{OliveGreen}1593.2 $\bm$ 265.0 &	\color{OrangeRed}731.1 $\bm$ 215.8 &	\color{MidnightBlue}173.5 $\bm$ 2.5 & 	171.1 $\bm$ 1.5	& 173.6 $\bm$ 2.4 &	\color{MidnightBlue}78.0 $\bm$ 166.6 &	\color{OrangeRed}-691.7 $\bm$ 801.0 & 	\color{OrangeRed}-141.8 $\bm$ 167.5\\
PPO     & \color{MidnightBlue}17.2 $\pm$ 84.4       & \color{OrangeRed}-113.3 $\pm$ 92.8   & \color{OrangeRed}-83.1 $\pm$ 117.7   & \color{OrangeRed}-28.0 $\pm$ 54.1      & \color{OrangeRed}-35.5 $\pm$ 87.8      & \color{MidnightBlue}163.4 $\pm$ 8.0     & 165.9 $\pm$ 15.4     & \color{OrangeRed}157.3 $\pm$ 12.6   & \color{MidnightBlue}86.5 $\pm$ 7.8      & \color{OliveGreen}120.5 $\pm$ 42.9     & \color{OliveGreen}120.3 $\pm$ 46.7   \\
TRPO    & \color{MidnightBlue}-12.0 $\pm$ 85.5      & \color{OrangeRed}-146.0 $\pm$ 67.4   & \color{OliveGreen}9.4 $\pm$ 57.6      & \color{OrangeRed}-32.7 $\pm$ 110.9     & \color{OrangeRed}-70.9 $\pm$ 71.9      & \color{MidnightBlue}166.7 $\pm$ 7.3     & 167.5 $\pm$ 6.7      & \color{OrangeRed}161.1 $\pm$ 13.0   & \color{MidnightBlue}47.3 $\pm$ 15.7     & \color{OrangeRed}-572.3 $\pm$ 368.0   & \color{OrangeRed}-818.0 $\pm$ 288.1 \\
TD3     & \color{MidnightBlue}3614.3 $\pm$ 82.1     & \color{OrangeRed}895.7 $\pm$ 61.6    & \color{OrangeRed}817.3 $\pm$ 11.0    & \color{OliveGreen}4256.5 $\pm$ 117.4    & \color{OliveGreen}3941.8 $\pm$ 61.3     & \color{MidnightBlue}161.4 $\pm$ 14.4    & \color{OliveGreen}169.2 $\pm$ 13.1     & \color{OliveGreen}170.2 $\pm$ 7.2    & \color{MidnightBlue}196.0 $\pm$ 3.1     &  \color{OrangeRed}190.4 $\pm$ 4.7      &  \color{OrangeRed}180.9 $\pm$ 8.2    \\
SAC     & \color{MidnightBlue}4000.7 $\pm$ 202.1    &  \color{OrangeRed}1146.7 $\pm$ 67.9   &  \color{OrangeRed}3869.2 $\pm$ 88.2   &  \color{OrangeRed}3530.5 $\pm$ 67.8     &  \color{OrangeRed}3708.1 $\pm$ 96.2     & \color{MidnightBlue}168.2 $\pm$ 9.5     & 169.3 $\pm$ 5.6      & 169.1 $\pm$ 12.6   & \color{MidnightBlue}199.4 $\pm$ 0.4     &  \color{OrangeRed}60.9 $\pm$ 23.4      &  \color{OrangeRed}70.7 $\pm$ 11.4   \\\bottomrule
\end{tabular}}
\vspace{0.1cm}
\caption{The performance of each algorithm in noisy environments.}\label{table:noisy_env}
\end{table}


%%%%% PREVIOUS %%%%%
% the dynamics are modelled with Gaussian processes
% We can denote the data matrix composed from data-set $\mathcal{D}$ as $\mathbf{X}, \,\mathbf{Y}$,
% and obtain the forward dynamics as $\tilde{f}_{\mathbf{X}, \mathbf{Y}} (s_t, a_t)$.
% Similarly we have the covariance as $\sigma_{\mathbf{X}, \mathbf{Y}} (s_t, a_t)$.
% The state distribution at every time-step can be written as $s_t\sim\rho(s_t | p(s_0), \mathbf{X}, \mathbf{Y}, \theta)$.
% To train the policy network, we directly take the gradient of the objective function with respect to the parameter of the policy network as
% $\theta_{i+1} = \theta_{i} + \alpha \frac{1}{\partial \theta_i}\partial\sum_0^{\infty}\mathbb{E}_{s_t\sim\rho}\left[r(s_t, a_t)\right]$.
%%%%%%%%



% We denote the state-action pair as $x_t \triangleq [s_t^T, a_t^T]^T$.
% The input and target data matrix for Gaussian process are defined respectively as $\mathbf{X} \triangleq [\{x_t\}]$, and $\mathbf{Y} \triangleq [\{s_{t+1} - s_{t}\}]$, where $(s_{t+1}, s_t, a_t)$ are all the data samples from $\mathcal{D}$.

%\begin{equation}
%    \begin{aligned}
%    \tilde{f}_{\mathbf{X}, \mathbf{Y}} (s_t, a_t) = s_t + k(\mathbf{X}, x_t)^{T}(K + \sigma_{\epsilon}^2I)^{-1}\mathbf{Y},
%    \end{aligned}
%\end{equation}
%$K$ is the Gram matrix, whose entry $K_{ij}$ is $k(x_i, x_j)$.
%\begin{equation}
%    \begin{aligned}
%    \theta_{i+1} = \theta_{i} - \alpha \frac{\partial \tilde{J}(\pi)}{\partial \theta_i} = \theta_{i} - \alpha \frac{1}{\partial \theta_i}\partial\mathbb{E}_{\theta_{i}, s_{t+1} \sim \mathcal{N}(\tilde{f}_{\mathbf{X}, \mathbf{Y}} (s_t, a_t), \sigma_{\mathbf{X}, \mathbf{Y}} (s_t, a_t))}\left[\sum_0^{\infty}r(s_t, a_t)\right].
%    \end{aligned}
%\end{equation}


% \ignasi{The part above is mine.}
% Here, the ground-truth dynamics are assumed to be known by the agent.
% The cost Q function can be written as $Q^i(s_i, a_{i:H}) = -\sum_{t=i}^{H} r(s_t, a_t)$,
% and the optimal value function can be written as $ V^i(s_i) = \min_{a_i} \left[-r(s_i, a_i) + Q^{i+1}(s_{i+1}, a_{i+1:H})\right]$ where $s_{i+1} = f (s_i, a_i)$.
%\begin{equation}
%    \begin{aligned}
%    Q^i(s_i, a_{i:\tau}) &= -\sum_{t=i}^{\tau} r(s_t, a_t), \\
%    V^i(s_i) &= \min_{a_i} \left[-r(s_i, a_i) + Q^{i+1}(s_{i+1}, a_{i+1:\tau})\right], \mbox{s.t.}\, s_{i+1} = f (s_i, a_i).
%    \end{aligned}
%\end{equation}
% By using dynamic programming,
% the optimal controller is a time-dependent linear controller.
% If we assume the change in state at time-step $i$ is $\delta s_i = s_i - \bar{s_i}$,
% the optimal controller is $a_i = \bar{a_i} + K(s_i - \bar{s_i})$, where $K$ is a feedback gain matrix.
% update is $\delta a_i = -Q_{a_i, a_i}^{i, -1}(Q_{a_i}+Q_{a_i, s_i}\delta s_i)$\jenny{Should we define the coefficients $Q_{aa}$, $Q_a$, $Q_{as}$?} \ignasi{Yes :), or not put them at all an just say that the optimal policy is a linear time-dependent policy that can be computed analytically}.
% In other words, we have a time-dependent local controller $a_i = \bar{a_i} + \pi(s_i - \bar{s_i})$.
% 
% Therefore, given the current trajectory $\{(s_t, a_t)\}$,
% we can update the action using the local controller $a_i' = a_i + \delta a_i$.
% In practice, MPC can be applied, where we only execute the first planned action, and update the future controllers based on the observed next state.
